Improved Measurements of Color-Suppressed Decays B0bar -> D0 pi0, D0 eta and D0 omega

We present preliminary improved measurements of the branching fractions of the color-suppressed decays B0bar -> D0 h0, where h0 represents the three light neutral mesons pi0, eta and omega. The measurements are based on a data sample of 140fb-1 collected at the Upsilon(4S) with the Belle detector at the KEKB energy-asymmetric e+e- collider, corresponding to seven times the luminosity of the previous Belle measurements.

==> defns.tex <==
%
% This is the input file required to accommodate
% the symbols used in that paper
% VT Oct 3 2003

\def\hb{\hfill\newline}

% Journals:

\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Journal definitions, no italics:
\def\EPJ{{Eur. Phys. Jour.} C}
\def\JMP{{Int. Jour. Mod. Phys.}}
\def\NCA{{Nuovo Cimento}}
\def\NIMA{{Nucl. Instr. Meth.} A}
\def\NPB{{Nucl. Phys. B\,}}
\def\PLB{{Phys. Lett.} B}
\def\PR{{Phys. Rev.}}
\def\PRD{{Phys. Rev.} D}
\def\PRL{{Phys. Rev. Lett.}}
\def\PRep{{Phys. Rep.}}
\def\PRepC{{Phys. Rep.} C}
\def\ZPC{{Z. Phys.} C}
\def\etal{{\it et al.}}

\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}
\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\FourS {\Y4S}
% Arrows
\RequirePackage{xspace}
\def\ra {\ensuremath{\rightarrow}\xspace}
% e+ e-
\def\epem {\ensuremath{e^+e^-}\xspace}
% P_T
\def\pt {\mbox{$p_T$}\xspace}
% BBbar
\def\BB {\ensuremath{B\Bbar}\xspace}
% qqbar
\def\qqbar {\ensuremath{q\overline q}\xspace}
% taup
\def\taup {\ensuremath{\tau^+}\xspace}
% nubar
\def\nub {\ensuremath{\overline{\nu}}\xspace}
% nubar_tau
\def\nutb {\ensuremath{\nub_\tau}\xspace}
% Monte Carlo
\newcommand{\mc}{{\rm Monte Carlo}}

\def\Kpi{\mbox{$\Kmi\pipl$}}
\def\Ktwopi{\mbox{$\Kmi\pipl\pizero$}}
\def\Kthreepi{\mbox{$\Kmi\pipl\pipl\pimi$}}
\def\ppeta{\mbox{$\pipl\pimi\eta$}}
\def\piS{\mbox{$\pi^0_S$}}
\def\piD{\mbox{$\pi^0_D$}}
\def\piH{\mbox{$\pi^0_H$}}
\def\etaM{\mbox{$\eta$}}
\def\etaPM{\mbox{$\eta^{\prime}$}}
\def\omegaM{\mbox{$\omega$}}
\def\De{\mbox{$\Delta E$}}
\def\Mb{\mbox{$M_{\rm bc}$}}
\def\Eb{\mbox{$E_{\rm beam}^{*}$}}
\def\mes{\mbox{$m_{\rm ES}$}}
\def\costhr{\mbox{$\cos{\theta_{\rm thr}}$}}
\def\cossph{\mbox{$\cos{\theta_{\rm sph}}$}}
\def\Acor{\mbox{${\cal A}_{\rm{corr}}$}}
\def\Bsec{\mbox{${\cal B}_{\rm sec}$}}
\def\Ncand{\mbox{${\cal N}_{\rm cand}$}}
\def\Pback{\mbox{${\cal N}_{\rm pb}$}}
\def\NPback{\mbox{${\cal N}_{\rm npb}$}}
\def\Ncf{\mbox{${\cal N}_{\rm CF}$}}

\providecommand{\thetathr}{\mbox{$\theta_{\rm thr}$}}
\providecommand{\thetasph}{\mbox{$\theta_{\rm sph}$}}
\providecommand{\thetahel}{\mbox{$\theta_{\rm hel}$}}
\providecommand{\thetadali}{\mbox{$\theta_{\rm D}$}}
\providecommand{\thetan}{\mbox{$\theta_{\rm N}$}}
\providecommand{\thetabst}{\mbox{$\theta_{\rm B^{\ast}}$}}

\def\stat{{\rm stat.}}
\def\syst{{\rm syst.}}

\providecommand{\rad}{\mbox{\rm rad}}
\providecommand{\psec}{\mbox{\rm ps}}
\providecommand{\fsec}{\mbox{\rm fs}}
\providecommand{\nsec}{\mbox{\rm nsec}}

\providecommand{\nm}{\mbox{\rm nm}}

\providecommand{\mum}{\mbox{$\rm \mu m$}}

\providecommand{\mm}{\mbox{\rm mm}}

\providecommand{\cm}{\,\mbox{\rm cm}}

\providecommand{\m}{\mbox{\rm m}}

\providecommand{\nb}{\mbox{\rm nb}}

\providecommand{\pb}{\mbox{\rm pb}}

\providecommand{\invpb}{\mbox{${\rm pb^{-1}}$}}
\providecommand{\invfb}{\mbox{${\rm fb^{-1}}$}}
\providecommand{\inch}{\mbox{\rm in}}
\providecommand{\eV}{\mbox{\rm eV}}
\providecommand{\keV}{\mbox{\rm keV}}
\providecommand{\MeV}{\,\mbox{\rm MeV}}
\providecommand{\MeVc}{\mbox{${\rm MeV}/c$}}
\providecommand{\MeVcsq}{\,\mbox{${\rm MeV}/c^2$}}
\providecommand{\GeV}{\,\mbox{\rm GeV}}
\providecommand{\GeVc}{\mbox{${\rm GeV}/c$}}
\providecommand{\GeVcsq}{\,\mbox{${\rm GeV}/c^2$}}
\providecommand{\dedx}{\mbox{$dE/dx$}}
\providecommand{\Br}{\mbox{${\cal B}$}}
\providecommand{\chisq}{\mbox{$\chi^2$}}
\providecommand{\ellpl}{\mbox{$\ell^+$}}
\providecommand{\ellmi}{\mbox{$\ell^-$}}
\providecommand{\nubar}{\mbox{$\overline{\nu}$}}
\providecommand{\nuel}{\mbox{$\nu_{\ell}$}}
\providecommand{\nuelbar}{\mbox{$\overline{\nu}_{\ell}$}}
\providecommand{\nue}{\mbox{$\nu_e}$}
\providecommand{\numu}{\mbox{$\nu_{\mu}$}}
\providecommand{\nutau}{\mbox{$\nu_{\tau}$}}
\providecommand{\epl}{\mbox{$e^+$}}
\providecommand{\emi}{\mbox{$e^-$}}
\providecommand{\eplemi}{\mbox{\epl \emi}}
\providecommand{\mupl}{\mbox{$\mu^+$}}
\providecommand{\mumi}{\mbox{$\mu^-$}}
\providecommand{\mupmum}{\mbox{\mupl\mumi}}
\providecommand{\hzero}{\mbox{$h^0$}}
\providecommand{\hmi}{\mbox{$h^-$}}
\providecommand{\Zzero}{\mbox{$Z^0$}}
\providecommand{\Wpl}{\mbox{$W^+$}}
\providecommand{\Wmi}{\mbox{$W^-$}}
\providecommand{\gamgam}{\gamma \gamma}
\providecommand{\pipl}{\mbox{$\pi^+$}}
\providecommand{\pimi}{\mbox{$\pi^-$}}
\providecommand{\pizero}{\mbox{$\pi^0$}}
\providecommand{\piplpimi}{\mbox{\pipl \pimi}}
\providecommand{\twopi}{\mbox{\pipl \pimi}}
\providecommand{\threepi}{\mbox{\pipl \pimi \pizero}}
\providecommand{\fourpi}{\mbox{\piplpimi\piplpimi}}
\providecommand{\etap}{\mbox{$\eta^\prime$}}
\providecommand{\rhopl}{\mbox{$\rho^+$}}
\providecommand{\rhomi}{\mbox{$\rho^-$}}
\providecommand{\rhozero}{\mbox{$\rho^0$}}
\providecommand{\rhop}{\mbox{$\rho(1450)$}}
\providecommand{\rhoprime}{\mbox{$\rho(1450)$}}
\providecommand{\neubar}{\mbox{$\overline{\nu}$}}
\providecommand{\neulbar}{\mbox{$\overline{\nu_{\ell}}$}}
\providecommand{\pbar}{\mbox{$\overline{p}$}}
\providecommand{\ppbar}{\mbox{$p \overline{p}$}}
\providecommand{\qbar}{\mbox{$\overline{q}$}}
\providecommand{\ubar}{\mbox{$\overline{u}$}}
\providecommand{\dbar}{\mbox{$\overline{d}$}}
\providecommand{\cbar}{\mbox{$\overline{c}$}}
\providecommand{\sbar}{\mbox{$\overline{s}$}}
\providecommand{\bbar}{\mbox{$\overline{b}$}}
\providecommand{\tbar}{\mbox{$\overline{t}$}}
\providecommand{\Kbar}{\kern 0.18em\overline{\kern -0.18em
K}{}\xspace} \providecommand{\Kzero}{\mbox{$K^0$}}
\providecommand{\Kzerobar}{\mbox{$\Kbar^0$}}
\providecommand{\Kpl}{\mbox{$K^+$}}
\providecommand{\Kmi}{\mbox{$K^-$}}
\providecommand{\KplKmi}{\mbox{$\Kpl\Kmi$}}
\providecommand{\KL}{\mbox{$K^0_L$}}
\providecommand{\KS}{\mbox{$K^0_S$}}
\providecommand{\KSKS}{\mbox{$\KS \KS$}}
\providecommand{\Kbar}{\mbox{$\overline{K}$}}
\providecommand{\KKbarpi}{\mbox{$K \Kbar \pi$}}
\providecommand{\Kstar}{\mbox{$K^*$}}
\providecommand{\Kstarpl}{\mbox{$K^{*+}$}}
\providecommand{\Kstarmi}{\mbox{$K^{*-}$}}
\providecommand{\Kstarzero}{\mbox{$K^{*0}$}}
\providecommand{\Ktwostar}{\mbox{$K_2^*(1430)$}}
\providecommand{\Lambdabar}{\mbox{$\overline{\Lambda}$}}
\providecommand{\Ecm}{\mbox{E_{CM}}}
\providecommand{\pt}{\mbox{p_T}}
\providecommand{\bbar}{\mbox{\bbar}}
\providecommand{\cbar}{\mbox{\cbar}}
\providecommand{\qbar}{\mbox{\qbar}}
%% CKM matrix elements:
\providecommand{\Vud}{\mbox{$V_{ud}$}}
\providecommand{\Vus}{\mbox{$V_{us}$}}
\providecommand{\Vub}{\mbox{$V_{ub}$}}
\providecommand{\Vcd}{\mbox{$V_{cd}$}}
\providecommand{\Vcs}{\mbox{$V_{cs}$}}
\providecommand{\Vcb}{\mbox{$V_{cb}$}}
\providecommand{\Vtd}{\mbox{$V_{td}$}}
\providecommand{\Vts}{\mbox{$V_{ts}$}}
\providecommand{\Vtb}{\mbox{$V_{tb}$}}
%% b -> u:
\providecommand{\btou}{\mbox{$b \to u$}}
%% b -> c:
\providecommand{\btoc}{\mbox{$b \to c$}}
% generic Dbar:
\providecommand{\Dbar}{\mbox{$\overline{D}$}}
% D0:
\providecommand{\Dzero}{\mbox{$D^0$}}
% D0bar
\providecommand{\Dzerobar}{\mbox{$\overline{D^0}$}}
% D+:
\providecommand{\Dpl}{\mbox{$D^+$}}
% D-:
\providecommand{\Dmi}{\mbox{$D^-$}}
% Ds:
\providecommand{\Ds}{\mbox{$D_s$}}
% Ds+:
\providecommand{\Dspl}{\mbox{$D_s^+$}}
% Ds-:
\providecommand{\Dsmi}{\mbox{$D_s^-$}}
% D*:
\providecommand{\Dstar}{\mbox{$D^{*}$}}
% D*+:
\providecommand{\Dstarpl}{\mbox{$D^{*+}$}}
% D*-:
\providecommand{\Dstarmi}{\mbox{$D^{*-}$}}
% D*0:
\providecommand{\Dstarzero}{\mbox{$D^{*0}$}}
% D*s:
\providecommand{\Dstars}{\mbox{$D^{*}_s$}}
% D*s+:
\providecommand{\Dstarspl}{\mbox{$D^{*+}_s$}}
% D*s-:
\providecommand{\Dstarsmi}{\mbox{$D^{*-}_s$}}
%D**:
\providecommand{\Dstarstar}{\mbox{$D^{**}$}}
%D(*)+:
\providecommand{\Dstpl}{\mbox{$D^{(*)+}$}}
%D(*)0:
\providecommand{\Dstze}{\mbox{$D^{(*)0}$}}
% B 
%\providecommand{\B}{\mbox{$\rm B\,$}}
\providecommand{\B}{\mbox{$B$\,}}
% Bbar:
\providecommand{\Bbar}{\kern 0.18em\overline{\kern -0.18em
B}{}\xspace}
% BBbar:
\providecommand{\BBbar}{\mbox{$B \Bbar$}}
% B0:
\providecommand{\Bzero}{\mbox{$B^0$}}
% B0bar:
\providecommand{\Bzerobar}{\mbox{$\Bbar^0$}}
% B+:
\providecommand{\Bpl}{\mbox{$B^+$}}
% B-:
\providecommand{\Bmi}{\mbox{$B^-$}}
% B0s:
\providecommand{\Bzeros}{\mbox{$B^0_s$}}
% B0d:
\providecommand{\Bzerod}{\mbox{$B^0_d$}}
% End of symbol file

%
 

